Large Scale Structure in Absorption: Gas within and around Galaxy Voids

We investigate the properties of the HI Ly-a absorption systems (Ly-a forest) within and around galaxy voids at z<0.1. We find a significant excess (>99% c.l.) of Ly-a systems at the edges of galaxy voids with respect to a random distribution, on ~5 h^{-1} Mpc scales. We find no significant difference in the number of systems inside voids with respect to the random expectation. We report differences between both column density (N_{HI}) and Doppler parameter (b_{HI}) distributions of Ly-a systems found inside and at the edge of galaxy voids at the >98% and >90% c.l. respectively. Low density environments (voids) have smaller values for both N_{HI} and b_{HI} than higher density ones (edges of voids). These trends are theoretically expected and also found in GIMIC, a state-of-the-art hydrodynamical simulation. Our findings are consistent with a scenario of at least three types of Ly-alpha: (1) containing embedded galaxies and so directly correlated with galaxies (referred as `halo-like'), (2) correlated with galaxies only because they lie in the same over-dense LSS, and (3) associated with under-dense LSS with a very low auto-correlation amplitude (~ random) that are not correlated with luminous galaxies. We argue the latter arise in structures still growing linearly from the primordial density fluctuations inside galaxy voids that have not formed galaxies because of their low densities. We estimate that these under-dense LSS absorbers account for 25-30% +- 6% of the current Ly-a population (N_{HI} > 10^{12.5} cm^{-2}) while the other two types account for the remaining 70-75% +- 12%. Assuming that only N_{HI} > 10^{14} cm^{-2} systems have embedded galaxies nearby, we have estimated the contribution of the `halo-like' Ly-a to be ~12-15% +- 4% and consequently ~55-60% +- 13% of the Ly-a systems to be associated with the over-dense LSS.

==> tabs/tab5.tex <==
\begin{table}
  \centering
  \begin{minipage}{80mm}
    \caption{Kolmogorov-Smirnov (KS) test probabilities between
      different \gimic~regions and our LSS samples\tablenotemark{a}.}\label{tab:4}
    \begin{tabular}{@{}c|rrrrr@{}}
  \hline
   \backslashbox{$N_{\rm HI}$}{$b_{\rm HI}$} 
             & $-2\sigma$   &$-1\sigma$   &  $0\sigma$  &$+1\sigma$ & $+2\sigma$     \\
  \hline                                                                               \\
  void
  edge
  \hline
  \end{tabular}
    \tablenotetext{a}{KS test probabilities for $\log N_{\rm HI}$ and
      \bhi~distributions are shown in the left-bottom and right-upper
      sides respectively.}
\end{minipage}
\end{table}



==> tabs/tab6.tex <==
\begin{table*}
  \centering
  \begin{minipage}{100mm}
    \caption{\hi~\lya~systems in our LSS samples\tablenotemark{a}.}\label{tab:6}
    \begin{tabular}{@{}lllcll@{}}
      \hline 

      Sight Line & $z_{\rm abs}$ & $X$ &$D$    & $\log(N_{HI}[\rm{cm}^{-2}])$ & $b_{HI}$ \\
                 &              &     &[\mpc] &                             &  [\kms] \\

      \hline


PG0953+414  &  0.0156  &  0.89 &  -1.6  &$13.14 \pm  0.07       $&$  35 \pm  6  $                     \\
PG0953+414  &  0.01603 &  0.89 &  -1.5  &$14.18 \ ^{+ \ 0.21}_{- \ 0.17} $&$  12 \ ^{+ \ 2}_{- \ 1}  $\\
PG0953+414  &  0.01655 &  0.91 &  -1.3  &$13.81 \ ^{+ \ 0.12}_{- \ 0.14} $&$  11 \ ^{+ \ 5}_{- \ 2}  $\\
PG0953+414  &  0.03054 &  0.69 &  -3.6  &$12.63 \ ^{+ \ 0.1}_{- \ 0.09}  $&$  14 \pm 14 $             \\
PG0953+414  &  0.04382 &  1.34 &  4.1   &$13.39 \ ^{+ \ 0.03}_{- \ 0.04} $&$  47 \pm 8  $             \\
PG0953+414  &  0.04469 &  1.19 &  2.2   &$12.77 \pm  0.05       $&$ 13 \pm 1  $                       \\
PG0953+414  &  0.04513 &  1.12 &  1.4   &$13.37 \pm  0.02       $&$ 36 \pm 1  $                       \\
PG0953+414  &  0.04623 &  0.97 &  -0.4  &$12.93 \pm  0.09       $&$ 20 \pm 2  $                       \\
PG0953+414  &  0.04782 &  0.87 &  -1.6  &$12.41 \pm  0.12       $&$ 19 \pm 6  $                       \\
PG0953+414  &  0.0496  &  0.95 &  -0.5  &$13.05 \pm  0.03       $&$ 26 \pm 2  $                       \\
PG0953+414  &  0.05876 &  1.07 &  1.0   &$13.92 \pm  0.09       $&$ 30 \ ^{+ \ 6}_{- \ 5}$            \\
PG0953+414  &  0.06808 &  1.22 &  3.2   &$14.46 \ ^{+ \ 0.18}_{- \ 0.14} $&$  21 \ ^{+ \ 3}_{- \ 2}  $\\
PG0953+414  &  0.09228 &  1.17 &  2.6   &$13.04 \ ^{+ \ 0.08}_{- \ 0.04} $&$  31 \pm  3 $             \\
PG0953+414  &  0.09315 &  1.3  &  4.5   &$13.67 \ ^{+ \ 0.03}_{- \ 0.09} $&$  31 \ ^{+ \ 17}_{- \ 9}$  \\
Ton28       &  0.01328 &  0.92 &  -1.1  &$12.94 \pm  0.1        $&$    13 \pm 3  $                    \\
Ton28       &  0.01533 &  1.04 &  0.6   &$14.17 \ ^{+ \ 0.35}_{- \ 0.34} $&$  25 \ ^{+ \ 21}_{- \ 7}$  \\
Ton28       &  0.02127 &  1.14 &  1.6   &$13.04 \pm  0.15       $&$ 14 \pm 4  $                       \\
Ton28       &  0.03357 &  0.68 &  -4.2  &$13.4  \pm  0.05       $&$ 75 \pm 7  $                       \\
Ton28       &  0.05123 &  1.4  &  5.7   &$13.14 \ ^{+ \ 0.09}_{- \ 0.08} $&$  46 \pm 46 $             \\
Ton28       &  0.06471 &  0.75 &  -5.2  &$13.38 \pm  0.09       $&$ 41 \pm 7  $                       \\
Ton28       &  0.077   &  0.74 &  -3.4  &$13.05 \pm  0.07       $&$ 13 \pm 2  $                       \\
Ton28       &  0.08978 &  0.94 &  -0.6  &$13.86 \pm  0.03       $&$ 30 \pm 1  $                       \\
Ton28       &  0.09295 &  1.12 &  1.4   &$13.89 \pm  0.08       $&$ 19 \pm 2  $                       \\
PG1116+215  &  0.01152 &  1.26 &  4.2   &$12.31 \pm  0.27       $&$ 12 \pm 10 $                       \\
PG1116+215  &  0.01639 &  1.02 &  0.3   &$13.44 \pm  0.03       $&$ 54 \pm 3  $                       \\
PG1116+215  &  0.02841 &  1.23 &  2.9   &$13.71 \ ^{+ \ 0.21}_{- \ 0.09} $&$ 43 \ ^{+ \ 24}_{- \ 23} $\\
PG1116+215  &  0.03234 &  1.43 &  5.3   &$13.29 \pm  0.03     $&$ 37 \pm 3 $                          \\
PG1116+215  &  0.04122 &  0.85 &  -1.5  &$13.13 \ ^{+ \ 0.06}_{- \ 0.05} $&$ 72 \pm 6  $              \\
PG1116+215  &  0.04995 &  0.7  &  -3.1  &$12.76 \pm  0.05     $&$ 15 \pm 2  $                         \\
PG1116+215  &  0.05904 &  1.22 &  2.7   &$13.53 \pm  0.02     $&$  45 \pm 1  $                        \\
PG1116+215  &  0.0608  &  0.92 &  -0.8  &$13.21 \pm  0.04     $&$  53 \pm 5  $                        \\
PG1116+215  &  0.06258 &  0.5  &  -5.5  &$13.1  \pm  0.06     $&$  65 \pm 7  $                        \\
PG1116+215  &  0.07535 &  0.55 &  -6.5  &$12.37 \pm  0.18     $&$  22 \pm 9  $                        \\
PG1116+215  &  0.08096 &  1.3  &  4.7   &$13.55 \ ^{+ \ 0.08}_{- \ 0.09} $&$  14 \ ^{+ \ 7}_{- \ 2}  $\\
PG1116+215  &  0.1     &  0.54 &  -5.6  &$12.89 \ ^{+ \ 0.06}_{- \ 0.05} $&$  22 \pm 22 $             \\
PG1211+143  &  0.01649 &  0.46 &  -7.4  &$13.52 \pm  0.02      $&$  36 \pm 1  $                       \\
PG1211+143  &  0.0168  &  0.44 &  -7.6  &$14.0  \ ^{+ \ 0.15}_{- \ 0.14} $&$  23 \ ^{+ \ 11}_{- \ 4}$  \\
PG1211+143  &  0.02206 &  1.13 &  1.8   &$13.27 \pm  0.02      $&$  24 \pm 1  $                       \\
PG1211+143  &  0.02335 &  1.4  &  5.4   &$13.46 \pm  0.02      $&$  35 \pm 1  $                       \\
PG1211+143  &  0.02422 &  1.5  &  6.2   &$12.23 \ ^{+ \ 0.27}_{- \ 0.16} $&$  20 \pm 20 $             \\
PG1211+143  &  0.02586 &  1.21 &  2.6   &$13.49 \pm  0.02      $&$  70 \pm 2  $                       \\
PG1211+143  &  0.02802 &  0.95 &  -0.6  &$12.27 \ ^{+ \ 0.11}_{- \ 0.16} $&$  20 \pm 7  $             \\
PG1211+143  &  0.03986 &  0.95 &  -0.9  &$12.59 \pm  0.08      $&$  36 \pm 7  $                       \\
PG1211+143  &  0.04521 &  1.23 &  2.3   &$13.05 \pm  0.02      $&$  32 \pm 1  $                       \\
PG1211+143  &  0.0456  &  1.15 &  1.5   &$12.47 \ ^{+ \ 0.12}_{- \ 0.05} $&$  23 \pm 4  $             \\
PG1211+143  &  0.05104 &  1.2  &  2.0   &$15.67 \ ^{+ \ 0.35}_{- \ 0.28} $&$  25 \ ^{+ \ 11}_{- \ 5}$  \\
PG1211+143  &  0.05145 &  1.22 &  2.8   &$14.13 \ ^{+ \ 0.11}_{- \ 0.2} $ &$  35 \pm 14 $             \\
PG1211+143  &  0.05205 &  1.25 &  3.2   &$13.58 \pm  0.04     $&$  42 \pm 4  $                        \\
PG1211+143  &  0.05443 &  1.08 &  1.1   &$13.19 \pm  0.03      $&$  98 \pm 1  $                       \\
PG1211+143  &  0.06447 &  1.22 &  2.4   &$15.73 \ ^{+ \ 0.32}_{- \ 0.12} $&$  18 \ ^{+ \ 1}_{- \ 2}  $\\
PG1211+143  &  0.06493 &  1.29 &  3.1   &$13.82 \ ^{+ \ 0.05}_{- \ 0.1} $&$  37 \ ^{+ \ 7}_{- \ 12} $ \\
PG1211+143  &  0.0654  &  1.36 &  3.9   &$12.97 \pm  0.09     $&$  27 \pm 2  $                        \\
PG1216+069  &  0.03777 &  1.58 &  7.5   &$13.58 \pm  0.19      $&$  38 \pm 17 $                       \\
PG1216+069  &  0.08047 &  1.48 &  5.9   &$13.87 \ ^{+ \ 0.28}_{- \ 0.1}  $&$  57 \ ^{+ \ 4}_{- \ 18} $\\     
\hline                    
    \end{tabular}         
    \tablenotetext{a}{$z_{\rm abs}$, \nhi~and \bhi~values come directly
      from the DS08 catalog. $X$ and $D$ are the distances to the closest
      void center and void-edge respectively, in $R_{\rm void}$ units
      (see \S \ref{gasaroundvoids} for further details).}
  \end{minipage}          
\end{table*}              
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          
                          


==> tabs/tab7.tex <==
\begin{table*}
  \centering
  \begin{minipage}{100mm}
    \caption{\hi~\lya~systems in our LSS samples (cont.)\tablenotemark{a}.}\label{tab:7}
    \begin{tabular}{@{}lllcll@{}}
      \hline 

      Sight Line & $z_{\rm abs}$ & $X$ & $D$     &  $\log(N_{HI}[\rm{cm}^{-2}])$ & $b_{HI}$ \\
                 &              &     &  [\mpc] &                              &  [\kms] \\

      \hline

3C273       &  0.02626 &  0.95 &  -0.9  &$12.95 \pm  0.02      $&$  28 \pm 1  $                             \\
3C273       &  0.02946 &  0.63 &  -6.4  &$13.7  \ ^{+ \ 0.03}_{- \ 0.04} $&$  13 \pm 1  $                   \\
3C273       &  0.0328  &  0.72 &  -4.9  &$12.83 \pm  0.03      $&$  24 \pm 1  $                             \\
3C273       &  0.03938 &  1.18 &  2.7   &$12.56 \ ^{+ \ 0.11}_{- \ 0.06} $&$  28 \pm 28 $                   \\
3C273       &  0.04664 &  0.99 &  -0.2  &$12.33 \ ^{+ \ 0.09}_{- \ 0.08} $&$  21 \pm 21 $                   \\
3C273       &  0.049   &  1.04 &  0.8   &$13.53 \ ^{+ \ 0.19}_{- \ 0.04} $&$  37 \ ^{+ \ 3}_{- \ 21} $      \\
3C273       &  0.04999 &  0.91 &  -1.9  &$12.85 \ ^{+ \ 0.04}_{- \ 0.03} $&$  25 \pm 2  $                   \\
3C273       &  0.06051 &  0.76 &  -5.1  &$12.22 \pm  0.08     $&$  18 \pm 3  $                              \\
3C273       &  0.06349 &  0.71 &  -4.2  &$13.05 \pm  0.02     $&$  28 \pm 1  $                              \\
3C273       &  0.06656 &  0.36 &  -9.3  &$14.17 \ ^{+ \ 0.11}_{- \ 0.15}$&$  31 \ ^{+ \ 13}_{- \ 5}  $      \\
3C273       &  0.07537 &  1.48 &  5.3   &$12.63 \ ^{+ \ 0.06}_{- \ 0.04}$&$  24 \pm 1  $                    \\
3C273       &  0.08764 &  1.09 &  1.0   &$13.05 \pm  0.02    $&$  42 \pm 2  $                               \\
3C273       &  0.0898  &  1.26 &  2.9   &$13.22 \ ^{+ \ 0.03}_{- \ 0.11}$&$  45 \ ^{+ \ 24}_{- \ 28} $      \\
3C273       &  0.09011 &  1.24 &  2.5   &$13.19 \pm  0.01    $&$  28 \pm 1  $                               \\
Q1230+0115  &  0.02516 &  1.06 &  1.0   &$13.09 \ ^{+ \ 0.05}_{- \ 0.08}$&$  28 \pm 5  $                    \\
Q1230+0115  &  0.02762 &  0.72 &  -4.8  &$12.64 \pm  0.09     $&$  11 \pm 3  $                              \\
Q1230+0115  &  0.04848 &  1.12 &  1.4   &$13.38 \pm  0.03      $&$  28 \pm 2 $                              \\
Q1230+0115  &  0.04886 &  1.1  &  1.2   &$13.05 \pm  0.05      $&$  17 \pm 2  $                             \\
Q1230+0115  &  0.07177 &  1.06 &  0.9   &$13.48 \pm  0.02      $&$  23 \pm 1  $                             \\
Q1230+0115  &  0.07805 &  1.29 &  3.1   &$15.06 \ ^{+ \ 0.4}_{- \ 0.04} $&$  23 \ ^{+ \ 2}_{- \ 4}  $       \\
Q1230+0115  &  0.08344 &  1.3  &  3.3   &$13.29 \ ^{+ \ 0.06}_{- \ 0.03} $&$  65 \pm 6  $                   \\
Q1230+0115  &  0.08479 &  1.05 &  0.5   &$13.4  \pm  0.02      $&$  23 \pm 1  $                             \\
Q1230+0115  &  0.0886  &  0.86 &  -1.6  &$13.55 \pm  0.02      $&$  37 \pm 1  $                             \\
Q1230+0115  &  0.1     &  1.25 &  3.5   &$13.17 \pm  0.05      $&$  61 \pm 8  $                             \\
PG1259+593  &  0.01502 &  0.92 &  -0.9  &$13.19 \pm  0.04      $&$  21 \pm 2  $                             \\
PG1259+593  &  0.02217 &  1.06 &  1.0   &$13.64 \ ^{+ \ 0.12}_{- \ 0.06} $&$  29 \ ^{+ \ 3}_{- \ 12} $      \\
PG1259+593  &  0.0425  &  1.26 &  3.9   &$12.91 \pm  0.08     $&$  23 \pm 3  $                              \\
PG1259+593  &  0.04606 &  0.69 &  -4.6  &$15.51 \ ^{+ \ 0.28}_{- \ 0.25} $&$  30 \ ^{+ \ 10}_{- \ 8}  $     \\
PG1259+593  &  0.0465  &  0.64 &  -5.4  &$14.75 \ ^{+ \ 0.38}_{- \ 0.22} $&$  16 \ ^{+ \ 18}_{- \ 5}  $     \\
PG1259+593  &  0.05256 &  0.98 &  -0.3  &$12.93 \ ^{+ \ 0.09}_{- \ 0.07} $&$  21 \pm 21 $                   \\
PG1259+593  &  0.05376 &  1.19 &  2.8   &$13.38 \pm  0.03      $&$  24 \pm 1  $                             \\
PG1259+593  &  0.06644 &  1.66 &  9.7   &$13.65 \ ^{+ \ 0.03}_{- \ 0.04} $&$  29 \ ^{+ \ 22}_{- \ 7}  $     \\
PG1259+593  &  0.06931 &  1.22 &  2.3   &$13.33 \pm  0.04     $&$  54 \pm 4  $                              \\
PG1259+593  &  0.08933 &  0.81 &  -2.4  &$14.05 \ ^{+ \ 0.1}_{- \ 0.14} $&$  26 \ ^{+ \ 11}_{- \ 4} $       \\
PG1259+593  &  0.09591 &  1.0  &   0    &$12.9  \pm  0.06     $&$  21 \pm 3  $                              \\
Mrk1383     &  0.01367 &  0.84 &  -2.9  &$13.17 \pm  0.06     $&$  44 \pm 6  $                              \\
Mrk1383     &  0.02362 &  1.18 &  3.2   &$13.14 \pm  0.06     $&$  21 \pm 3  $                              \\
Mrk1383     &  0.02446 &  1.3  &  5.4   &$12.94 \ ^{+ \ 0.07}_{- \ 0.06} $&$  24 \pm 4  $                   \\
Mrk1383     &  0.02822 &  1.57 &  6.6   &$13.67 \pm  0.21     $&$  36 \pm 21 $                              \\
Mrk1383     &  0.03416 &  0.99 &  -0.1  &$12.71 \pm  0.11      $&$  28 \pm 7  $                             \\
Mrk1383     &  0.03752 &  1.29 &  3.6   &$13.09 \pm  0.06      $&$  26 \pm 3  $                             \\
Mrk1383     &  0.05184 &  1.24 &  2.8   &$14.16 \ ^{+ \ 0.17}_{- \ 0.14} $&$  26 \ ^{+ \ 10}_{- \ 4} $      \\
Mrk1383     &  0.05537 &  1.57 &  7.5   &$12.72 \ ^{+ \ 0.15}_{- \ 0.06} $&$  20 \ ^{+ \ 2}_{- \ 2} $       \\
Mrk1383     &  0.06734 &  0.6  &  -8.0  &$12.77 \ ^{+ \ 0.09}_{- \ 0.05} $&$  48 \ ^{+ \ 1}_{- \ 1}  $      \\
Mrk1383     &  0.06796 &  0.64 &  -7.1  &$12.45 \pm  0.08     $&$  12 \pm 2  $                              \\
Mrk1383     &  0.07938 &  1.4  &  4.6   &$12.61 \pm  0.06     $&$  31 \pm 4  $                              \\
Mrk1383     &  0.08345 &  1.76 &  8.7   &$13.08 \pm  0.03     $&$  20 \pm 1  $                              \\
Mrk1383     &  0.08442 &  1.73 &  7.4   &$12.94 \pm  0.07     $&$  32 \pm 7  $                              \\
PG1444+407  &  0.0188  &  0.98 &  -0.2  &$13.39 \pm  0.04     $&$  37 \pm 3  $                              \\
PG1444+407  &  0.02744 &  1.31 &  4.2   &$13.58 \pm  0.03     $&$  39 \pm 2  $                              \\
PG1444+407  &  0.09534 &  0.89 &  -1.7  &$13.89 \pm  0.03     $&$  26 \pm 1  $                              \\
PG1444+407  &  0.09586 &  0.92 &  -1.3  &$13.75 \pm  0.03     $&$  30 \pm 2  $                              \\  
    
\hline
    \end{tabular}
    \tablenotetext{a}{$z_{\rm abs}$, \nhi~and \bhi~values come directly
      from the DS08 catalog. $X$ and $D$ are the distances to the closest
      void center and void-edge respectively, in $R_{\rm void}$ units
      (see \S \ref{gasaroundvoids} for further details).}
  \end{minipage}
\end{table*}

